OCTen: Online Compression-based Tensor Decomposition

Tensor decompositions are powerful tools for large data analytics as they jointly model multiple aspects of data into one framework and enable the discovery of the latent structures and higher-order correlations within the data. One of the most widely studied and used decompositions, especially in data mining and machine learning, is the Canonical Polyadic or CP decomposition. However, today's datasets are not static and these datasets often dynamically growing and changing with time. To operate on such large data, we present OCTen the first ever compression-based online parallel implementation for the CP decomposition. We conduct an extensive empirical analysis of the algorithms in terms of fitness, memory used and CPU time, and in order to demonstrate the compression and scalability of the method, we apply OCTen to big tensor data. Indicatively, OCTen performs on-par or better than state-of-the-art online and online methods in terms of decomposition accuracy and efficiency, while saving up to 40-200 % memory space.

==> 021preliminaries.tex <==
\section{Preliminaries}
\label{sec:prelim}
\subsection{Definitions}
\textbf{Tensor} : A tensor is a higher order generalization of a matrix. An $N$-mode tensor is essentially indexed by $N$ variables. In particular, regular matrix with two variables i.e. $I$ and $J$ is 2-mode tensor, whereas data cube ( $I$,$J$ and $K$) is viewed as a 3-mode tensor $\tensor{X} \in \mathbb{R}^{I\times J \times K} $.
The number of modes is also called "order". Table \ref{table:t2} contains the symbols used throughout the paper. For the purposes of background explanation, we refer the reader to \cite{papalexakis2016tensors} for the definitions of Khatri-Rao and Kronecker products which are not necessary for understanding the basic derivation of our framework.
\hide{A tensor is a higher order generalization of a matrix. In order to avoid overloading the term ``dimension'', we call an $I\times J \times K$ tensor a three ``mode'' tensor, where ``modes'' are the numbers of indices used to index the tensor. The number of modes is also called ``order''. Table \ref{table:t2} contains the symbols used throughout the paper. In the interest of space, we also refer the reader to \cite{papalexakis2016tensors} for the definitions of Kronecker and Khatri-Rao products which are not necessary for following the basic derivation of our method. }

\textbf{Slice} :  A slice is a (N-1)-dimension partition of tensor $\tensor{X}$ where size is varied only in temporal mode and other non-temporal modes remain fixed.
% %***************************Table***************************
\begin{table}[h!]
	\small
	\begin{center}
		
		\begin{tabular}{ c lc }
			\hline
			\textbf{Symbols} & \textbf{Definition} \\ 
			\hline
			\hline
			$\tensor{X}$  & a tensor  \\ 
			$\mathbf{X}$ & a matrix (uppercase, bold letter) \\
			$ \mathbf{x} $ & a column vector  (lowercase, bold letter)\\
			$ x$ & a scalar (lowercase, italic letter) \\
			$\mathbf{X}^{(n)}$ &	mode-n matricization of a tensor\\
			$R$ & number of components\\
			$\mathbb{R}$ & set of Real Numbers  \\ 
			$\circ$ & outer product  \\ 
			$\oplus$&  a summation \\ 
			$\otimes $& Kronecker product\cite{papalexakis2016tensors}\\
			$\odot$ & Khatri-Rao product\cite{papalexakis2016tensors}\\
			$\mathbf{X}^T$ & a transpose of matrix $\mathbf{X}$ \\
			$\lVert \mathbf{X} \rVert_F$& Frobenius norm of $\mathbf{X}$  \\
			$nnz(\tensor{X}) $ & number of nonzero elements   of $\tensor{X}$ \\
			$I, J, K$&  dimensions of 3-mode of input tensor $\tensor{X}$\\
			$R, R, R$& dimensions of 3-mode of core tensor$\tensor{G}$\\
			
			\hline
		\end{tabular}
		\caption{\bf{Table of symbols and their description}}
		\label{table:t2}
	\end{center}
	
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Outer product}. We use $\circ$ to denote the outer product. The 3-mode outer product of vectors $\mathbf{a} \in \mathbb{R}^I , \mathbf{b} \in \mathbb{R}^J , and \mathbf{c} \in \mathbb{R}^K$, is a tensor $\tensor{X}= \mathbf{a} \circ \mathbf{b} \circ \mathbf{c}$ whose element (i, j, k) is defined as $\mathbf{a} \circ \mathbf{b} \circ \mathbf{c}_{ijk}=a_ib_jc_k$. 

\textbf{Kronecker product}. The Kronecker product of matrices $\mathbf{X}$ and $\mathbf{Y}$ of size IR and JR respectively, generates a matrix of size $I^2 R^2$, which can be defined as:
$$\mathbf{X} \otimes \mathbf{Y}=
\begin{bmatrix}
	  x_{11}\mathbf{Y} \ \ x_{12}\mathbf{Y} \dots  x_{1R}\mathbf{Y} \ \  \\
	  x_{21}\mathbf{Y} \ \ x_{22}\mathbf{Y} \dots  x_{2R}\mathbf{Y} \\
	\dots\\
	  x_{I1}\mathbf{Y} \ \ x_{I2}\mathbf{Y} \dots  x_{IR}\mathbf{Y} \\
\end{bmatrix}
$$
\textbf{Khatri-Rao product}. The Khatri-Rao product or column-wise Kronecker product of matrices $\mathbf{X}$ and $\mathbf{Y}$ that have the same number of columns, say R, is defined as:
$$\mathbf{X} \odot \mathbf{Y} = [\mathbf{x}(:,1) \otimes \mathbf{y}(:,1)  \mathbf{x}(:,2) \otimes \mathbf{y}(:,2) ··· \mathbf{x}(:,R) \otimes \mathbf{y}(:,R)]$$
If the sizes of $\mathbf{X}$ and $\mathbf{Y}$ are I-by-R and J-by-R, respectively, then $\mathbf{X} \odot \mathbf{Y}$ is IJ-by-R.

\textbf{Tensor rank}. The rank of a 3-mode tensor	$\tensor{X}$ is the smallest integer R such that there exist R rank-1 tensors whose sum is equal to the tensor 	$\tensor{X}$, i.e.,
$$\tensor{X} = \sum_{r=1}^{R} \mathbf{a} \circ \mathbf{b} \circ \mathbf{c}$$

\subsection{Tensor Decomposition} 
Tensor decomposition is a general tool for tensor analysis. Using tensor decomposition, we find latent factor or relations within data. There are two major tensor decompositions i.e. CP and Tucker.  In this paper, we focus on most popular CP tensor decompositions.

\textbf{Canonical Polyadic(CP) Decomposition for N-mode tensors}: One of the most popular and extensively used tensor decompositions is the Canonical Polyadic (CP) or CANDECOMP/ PARAFAC decomposition  \cite{carroll1970analysis,PARAFAC,bader2015matlab} referred as CP decomposition. Given a N-mode tensor $\tensor{X}$ of dimension $\mathbb{R}^{I_1 \times I_2\times \dots I_N}$, its CP decomposition can be written as $\mathbf{A}^{(n)} \in \mathbb{R}^{I_n \times R}$, where $n=(1,2,\dots N)$ and R represents the number of latent factors or upper bound rank on tensor $\tensor{X}$. Henceforth, the 3-mode tensor of size $\mathbb{R}^{I  \times J\times K}$ can be represented as a sum of rank-one tensors:
$
\tensor{X} \thickapprox \sum_{r=1}^R \mathbf{A}(:,r) \circ \mathbf{B}(:,r)\circ \mathbf{C}(:,r)
$
where $\mathbf{A}\in  \mathbb{R}^{I\times R}, \mathbf{B}\in \mathbb{R}^{J \times R},  \mathbf{C}\in \mathbb{R}^{K\times R}$. The unfold n-mode tensor $\tensor{X}$ can be written as khari-rao product of its modes as 
$
\tensor{X}^{(n)} \thickapprox   \mathbf{A}^{(n)} (\mathbf{A}^{(N)} \dots \odot \mathbf{A}^{(n+1)} \odot \mathbf{A}^{(n-1)} \odot \mathbf{A}^{(1)})^T  
$.

Figure \ref{fig:cp3way} shows the 3-way CP tensor decomposition.
\begin{figure}[!ht]
	\begin{center}
		\includegraphics[clip,trim=3cm 4cm 1.5cm 3cm,width = 0.45\textwidth]{FIG/cp3way.pdf}
		\caption{\bf{Rank-R CP decomposition of a 3-mode tensor. The tensor $\tensor{X}$  of dimension $\mathbb{R}^{I  \times J\times  K}$ is decomposed as three factor matrices $\mathbf{A}\in  \mathbb{R}^{I\times R}, \mathbf{B}\in \mathbb{R}^{J \times R},$ and  $\mathbf{C}\in \mathbb{R}^{K\times R}$. The small tensor $\tensor{g}$ of dimension $\mathbb{R}^{R  \times R\times  R}$ is super diagonal and each diagonal element value is equal to 1. }}
		\label{fig:cp3way}
	\end{center}
\end{figure}
	
\textbf{CP-ALS.} Algorithm \ref{alg:cpalsalg} shows the alternating least squares (ALS) algorithm for 3-mode CP decomposition.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% Algorithm %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{center}
	%\vspace{-0.25in}
	\begin{algorithm} [!htp]
		\small
		\caption{3-mode CP-ALS tensor decomposition}
		\begin{algorithmic}
			\REQUIRE $\tensor{X} \in \mathbb{R}^{I \times J \times K}$, max iterations $T$.
			
			\ENSURE Factor matrices $\mathbf{A}\in  \mathbb{R}^{I\times R}, \mathbf{B}\in \mathbb{R}^{J \times R},$  $\mathbf{C}\in \mathbb{R}^{K\times R}$, $\mathbf{\lambda} \in \mathbb{R}^{R}$.
			
			\While{$iter \leftarrow 1$ to $T$ and convergence tolerance} 
			{
				\STATE Initialize $\mathbf{A}$, $\mathbf{B}$, $\mathbf{C}$; \\
				\STATE $\mathbf{A} \leftarrow \mathbf{X}^{(1)} (\mathbf{C} \odot \mathbf{B}) (\mathbf{C}^T \mathbf{C} * \mathbf{B}^T \mathbf{B})$;\\
				\STATE $\mathbf{\lambda} \leftarrow norm(\mathbf{A})$;\\
			    \STATE $\mathbf{B} \leftarrow \mathbf{X}^{(2)} (\mathbf{C} \odot \mathbf{A}) (\mathbf{C}^T \mathbf{C} * \mathbf{A}^T \mathbf{A})$;\\
			    \STATE $\mathbf{\lambda} \leftarrow \lambda * norm(\mathbf{B})$;\\
			    \STATE $\mathbf{C} \leftarrow \mathbf{X}^{(3)} (\mathbf{B} \odot \mathbf{A}) (\mathbf{B}^T \mathbf{B} * \mathbf{A}^T \mathbf{A})$;\\
			    \STATE $\mathbf{\lambda} \leftarrow \mathbf{\lambda} * norm(\mathbf{C})$;\\
			    \STATE $\mathcal{L}  \approx \min||\tensor{X}^{(n)} -  \lambda (\mathbf{A} \odot \mathbf{B}  \odot \mathbf{C})||_F^2
			    $
		}					
		 \RETURN ($\mathbf{A},\mathbf{B},\mathbf{C},\mathbf{\lambda}$)
		\end{algorithmic}
		\label{alg:cpalsalg}
	\end{algorithm}
	%	\vspace{-0.1in}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We refer the interested reader to several well-known surveys that provide more details on tensor decompositions and its applications \cite{kolda2009tensor,papalexakis2016tensors}.
